Sparse Quantile Huber Regression for Efficient and Robust Estimation

We consider new formulations and methods for sparse quantile regression in the high-dimensional setting. Quantile regression plays an important role in many applications, including outlier-robust exploratory analysis in gene selection. In addition, the sparsity consideration in quantile regression enables the exploration of the entire conditional distribution of the response variable given the predictors and therefore yields a more comprehensive view of the important predictors. We propose a generalized OMP algorithm for variable selection, taking the misfit loss to be either the traditional quantile loss or a smooth version we call quantile Huber, and compare the resulting greedy approaches with convex sparsity-regularized formulations. We apply a recently proposed interior point methodology to efficiently solve all convex formulations as well as convex subproblems in the generalized OMP setting, pro- vide theoretical guarantees of consistent estimation, and demonstrate the performance of our approach using empirical studies of simulated and genomic datasets.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX= pdflatex
BIBTEX= bibtex
FIG2DEV=fig2dev

TEX=ElasticCheck.tex \
		Abstract.tex \
		Introduction.tex \
		Formulation.tex \
		OMP.tex \
		Optimization.tex \
		Experiments.tex \
		Asymptotics.tex \
		robust.bib

all: pdf 

pdf: $(TEX) ElasticCheck.bbl
	@echo Compiling ElasticCheck
	@$(LATEX) ElasticCheck
	@$(MAKE) fixlabels

fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' ElasticCheck.log),0)
	@echo Compiling ElasticCheck again to fix labels
	@$(LATEX) ElasticCheck
else
	@echo " " Labels are correct
endif

ElasticCheck.bbl: robust.bib
	@echo Compiling ElasticCheck for bibliography
	@$(LATEX) ElasticCheck
	@echo Generating bibliography
	@$(BIBTEX) ElasticCheck
	@echo Recompiling ElasticCheck after generating bibliography
	@$(LATEX)  ElasticCheck
	@$(MAKE) fixlabels

.eps.pdf:
	@echo " " Converting $< to $(@F)
	@epstopdf --outfile=Figs/$(@F) $<

clean:
	@echo "Cleaning the figures directory"
	@rm -f figures/*.gpl
	@echo "Cleaning the ElasticCheck directory"
	@rm -f ElasticCheck.pdf ElasticCheck.ps *.aux *.dvi *.log *.bbl *.blg *.toc *.out *.bak


==> OldStuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\ell_1$ penalized version via ADMM}
We can solve using the Alternating Direction  Method of Multipliers (ADMM) as follows.  (The original quantile regression and LAD lasso have been solved traditionally using linear programing and interior point methods. But these suffer from convergence issues and do not scale to ultra high dimensional problems. )

For absolute loss ($\tau=0.5$) we have:
%
\begin{algorithm}\label{algorithm}\caption{$\ell_1$-penalized Elastic-Check: ADMM solver}\small
\noindent

{\bf Initialization:} $k=0,  \beta^{0}=\mathbf{0}_p, z^{0}=\mathbf{0}_n, u^{0}=\mathbf{0}_n$\\
{\bf Repeat}: 
\begin{align}
	&\beta^{k+1}:=\arg\min_\beta \left( \lambda\|\beta\|_1 + (\rho/2)\|-X\beta+(y-z^{k}+u^{k})\|_2^2\right)\label{eq::prox}\\
	&z^{k+1}:=\arg\min_z \left((1-\alpha)\|z\|_1 + \frac{\alpha}{2} \|z\|_2^2 + (\rho/2)\|-X\beta+(y-z^{k}+u^{k})\|_2^2\right)\\
&\qquad=S_{(1-\alpha)/(\alpha+\rho)}(\frac{\rho}{\alpha+\rho}(u+y-X\beta))\label{eq::thresh}\\
        &u^{k+1}:=u^{k}+y-X\beta^{k+1}-z^{k+1}\nonumber\\
	&k:=k+1\nonumber
\end{align}
{\bf Until Convergence.}
\end{algorithm}

The proximal step of (\ref{eq::prox}) is a Lasso problem which can be solved using glment or ADMM or FISTA or any other method.

$S$ in \eqref{eq::thresh} is the \emph{soft-thresholding operator} defined as
\begin{equation} \label{eq::soft_thresholding}
S_{\kappa}(a)=\left\{ \begin{array}{ll}
a-\kappa & a>\kappa\\
0 & |a| <\kappa\\
a+\kappa & a< -\kappa\\
\end{array}
\right.
\end{equation}


For more general quantiles, the soft thresholding step has to be replaced by
\[
 \arg\min_z \left((1-\alpha)c_{\tau}(z) + \frac{\alpha}{2} \|z\|_2^2 + (\rho/2)\|-X\beta+(y-z^{k}+u^{k})\|_2\right)\\
\]

Things are separable again, and for each coordinate $z_i$, we can apply a generalized form of thresholding 
\begin{equation}
S_{\kappa}(a)=\left\{ \begin{array}{ll}
a -\frac{\kappa}{\rho} \tau & a>\frac{\kappa}{\rho} \tau \\
0 & a \in \frac{\kappa}{\rho}[-(1-\tau),\tau]\\
a+\frac{\kappa}{\rho}  (1-\tau) & a< - \frac{\kappa}{\rho}  (1-\tau)\\
\end{array}
\right.
\end{equation}

Instead of the ADMM approach, one can consider smoothing of the check function and apply FISTA (FISTA works well when one has 1 smooth and 1 non-smooth function, but not 2!). The expected numerical convegence rate is $1/k,$ where $k$ is the iteration, as we pay a price for smoothing.


\textbf{[Open question:  Note however that the 2 non-smooth functions in our objective function are of similar nature, so it may be able to combine them somehow within FISTA.] }
\red{Ronny: Could you please add the details of the smoothing you derived? Thanks!}

\textbf{[TODO:  Once we have all the methods, we should compare numerical convergence, timing]}

\subsection{$\ell_1$ penalized version via smoothing}
We are again interested in solving the $\ell_1$ penalized problem (\ref{equ::penalized-loss}).  Rather than apply ADMM, we here smooth the check function and optimize the resulting problem consisting of a smooth loss with $\ell_1$ penalty.  Define
\[\begin{array}{ll}
C_\tau(\beta)&=\sum_i{c_\tau(y_i-X_i'\beta)}\\
&=\sum_i{\max{\{u_i(y_i-X_i'\beta): -(1-\tau)\leq u_i\leq\tau, u_i\in\scrR\}}}\\
&=\max{\{\langle u,y-X\beta\rangle :-(1-\tau)\leq u\leq\tau, u\in\scrR^n\}}
\end{array}
\]
In relating to \cite{Nest2003}, define
\[
Q=\{u : -(1-\tau)\leq u\leq\tau\},
\]
\[
\hat{\phi}(u)=-y'u,
\]
and 
\[
d(u)=\frac{1}{2}\|u\|_2^2,
\]
where $d(u)$ has strong convexity paramter $\sigma=1$.  We define the smooth approximation to $C_\tau(\beta)$ as
\[\begin{array}{ll}
C_\tau^\mu(\beta)&=\max_{u\in Q}{\{\langle-X\beta,u\rangle-\hat{\phi}(u)-\mu d(u)\}}\\
&=\max_{u\in Q}{\{\langle-X\beta+y,u\rangle-\frac{1}{2}\|u\|_2^2\}}.
\end{array}\]
Let 
\[\begin{array}{ll}
u_\mu(\beta)&=\arg\max_{u\in Q}{-\frac{1}{2}\mu\big(u'u-2\langle\frac{-X\beta+y}{\mu},u\rangle\big)}\\
&=P_Q\big(\frac{-X\beta+y}{\mu}\big).
\end{array}\]
The gradient of $C^\mu_\tau(\beta)$ is given by
\[
\nabla C^\mu_\tau(\beta)=-X'u_\mu(\beta)
\]
 and can be shown to be lipschitz continuous with lipschitz constant $L_\mu=\|X\|_F^2/\mu\sigma$. Define $D=\max{\{\|u\|^2_2/2 : u\in Q\}}$.  Then we can bound the nonsmooth check function $C_\tau(\beta)$ by
\[
C^\mu_\tau(\beta) \leq C_\tau(\beta) \leq C^\mu_\tau(\beta) + \mu D.
\]
Now, rather than solve the original problem (\ref{equ::penalized-loss}), we solve the following problem that has only one nonsmooth term:
\[\begin{array}{ll}
\beta(\mu)&=\arg\min{\{(1-\alpha)C_\tau^\mu(\beta)+\frac{\alpha}{2}\|y-X\beta\|^2_2+\lambda\|\beta\|_1\}}\\
&=\arg\min{\{L_\alpha^\mu(\beta)+\lambda\|\beta\|_1\}},
\end{array}\]
with $L_\alpha^\mu(\beta)=(1-\alpha)C_\tau^\mu(\beta)+\frac{\alpha}{2}\|y-X\beta\|^2_2$.  In order to see how solving this approximated problem leads to a solution of the original problem, denote $g_\alpha^\mu(\beta)=L^\mu_\alpha(\beta)+\lambda\|\beta\|_1$ and $g_\alpha(\beta)=L_\alpha(\beta)+\lambda\|\beta\|_1$.  Using the approximation to $C_\tau^\mu(\beta)$, we have the following relationship for any $\beta$:
\[\begin{array}{ll}
g_\alpha(\beta)-g_\alpha(\beta^*)&\leq g^\mu_\alpha(\beta)-g_\alpha(\beta^*)+(1-\alpha)\mu D\\
&\leq g^\mu_\alpha(\beta)-g^\mu_\alpha(\beta^*)+(1-\alpha)\mu D\\
&\leq g^\mu_\alpha(\beta)-g^\mu_\alpha(\beta(\mu))+(1-\alpha)\mu D.
\end{array}\]
If we solve the approximate problem with a $\beta$ that satisfies 
\[
g^\mu_\alpha(\beta)-g^\mu_\alpha(\beta(\mu))+(1-\alpha)\mu D\leq\epsilon
\]
and choose $\mu=\epsilon/(2(1-\alpha)D)$, then this $\beta$ that is $\epsilon/2$ optimal for the approximate problem is $\epsilon$ optimal for the original problem (\ref{equ::penalized-loss}).  Regarding the convergence rate, the proof in \cite{Beck2009} shows that $\epsilon/2$ optimality of $g^\mu_\alpha(\beta)$ can be reached in 
\[
\frac{2\sqrt{L(g^\mu_\alpha)}\|\beta_0-\beta(\mu)\|_2}{\sqrt{\epsilon}}
\]
iterations where $\beta_0$ is the initial point in the algorithm and $L(g^\mu_\alpha)$ is the lipschitz constant of $g^\mu_\alpha(\beta)$.  Since $L(g^\mu_\alpha)=(1-\alpha)\|X\|_F^2/\mu+\alpha\|X\|_F=2(1-\alpha)^2\|X\|_F^2D/\epsilon+\alpha\|X\|_F$, so that $\epsilon$ optimality of the true objective $g_\alpha(\beta)$ can be reached in 
\[
\frac{2\sqrt{2D}(1-\alpha)\|X\|_F\|\beta_0-\beta(\mu)\|_2}{\epsilon}+\frac{2\sqrt{\alpha\|X\|X\|_F}\|\beta_0-\beta(\mu)\|_2}{\sqrt{\epsilon}}
\]
iterations.  The first term dominates implying that the algorithm converges at a rate $O(1/k)$.  The algorithm applied here is FISTA and given by Algorithm \ref{algorithm::FISTA}. The projection step is given by
\[
p_L(\gamma)=\arg\min_\beta{\big\{\lambda\|\beta\|_1+\frac{L(g^\mu_\alpha)}{2}\big\|\beta-(\gamma-\frac{1}{L(g^\mu_\alpha)}(-(1-\alpha)X'u_\mu(\gamma)-\alpha X'(y-X\gamma))\big\|_2^2\big\}}
\]
which can be solved in closed form by the soft thresholding formula (\ref{eq::soft_thresholding}). 

\begin{algorithm}\label{algorithm::FISTA}\caption{$\ell_1$-penalized Elastic-Check: FISTA solver}\small
\noindent

{\bf Initialization:} $L=L(g^\mu_\alpha), \beta^0=\mathbf{0}_p, \gamma^1=\beta^0, t_1=1,k=1$\\
{\bf Repeat}: 
\begin{align}
& \beta^k=p_L(\gamma^k)\\
& t_{k+1}=\frac{1+\sqrt{1+4t_k^2}}{2}\\
& \gamma^{k+1}=\beta^k+\big(\frac{t_k-1}{t_{k+1}}\big)(\beta^k-\beta^{k-1})\\
& k:=k+1\nonumber
\end{align}
{\bf Until Convergence.}
\end{algorithm}

 

